Sound Probabilistic #SAT with Projection

We present an improved method for a sound probabilistic estimation of the model count of a boolean formula under projection. The problem solved can be used to encode a variety of quantitative program analyses, such as concerning security of resource consumption. We implement the technique and discuss its application to quantifying information flow in programs.

==> eptcsdata.tex <==
\providecommand{\firstpage}{15}
\providecommand{\publicationstatus}{M. Tribastone and H. Wiklicky (Eds.): International Workshop on\\Quantitative Aspects of Programming Languages and Systems (QAPL'16)\\
EPTCS 227, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.227.2}{10.4204/EPTCS.227.2}}
\pdfoutput=1

